Economics of Spot Instance Service: A Two-stage Dynamic Game Apporach

This paper presents the economic impacts of spot instance service on the cloud service providers (CSPs) and the customers when the CSPs offer it along with the on-demand instance service to the customers. We model the interaction between CSPs and customers as a non-cooperative two-stage dynamic game. Our equilibrium analysis reveals (i) the techno-economic interrelationship between the customers' heterogeneity, resource availability, and CSPs' pricing policy, and (ii) the impacts of the customers' service selection (spot vs. on-demand) and the CSPs' pricing decision on the CSPs' market share and revenue, as well as the customers' utility. The key technical challenges lie in, first, how we capture the strategic interactions between CSPs and customers, and second, how we consider the various practical aspects of cloud services, such as heterogeneity of customers' willingness to pay for the quality of service (QoS) and the fluctuating resource availability. The main contribution of this paper is to provide CSPs and customers with a better understanding of the economic impact caused by a certain price policy for the spot service when the equilibrium price, which from our two-stage dynamic game analysis, is able to set as the baseline price for their spot service.

==> background.tex <==
\section{Background}






---------------------------------
\vspace{1cm}




{\color{black}
Game theory and two-stage dynamic game based analysis




}

%\vspace{5cm}
